Rescan: Inductive Instance Segmentation for Indoor RGBD Scans

In depth-sensing applications ranging from home robotics to AR/VR, it will be common to acquire 3D scans of interior spaces repeatedly at sparse time intervals (e.g., as part of regular daily use). We propose an algorithm that analyzes these "rescans" to infer a temporal model of a scene with semantic instance information. Our algorithm operates inductively by using the temporal model resulting from past observations to infer an instance segmentation of a new scan, which is then used to update the temporal model. The model contains object instance associations across time and thus can be used to track individual objects, even though there are only sparse observations. During experiments with a new benchmark for the new task, our algorithm outperforms alternate approaches based on state-of-the-art networks for semantic instance segmentation.

==> figures/fullvslimitedmovement.tex <==
% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=0.5\textwidth]{images/full_vs_limited_comparison.jpg}
%     \captionof{figure}{A qualitative comparison of full vs limited movement schemes. (a) is the source scene with instance segmentation. (b) is the target scene visualization. (c) and (d) show result using our method using limited movement and result using full version of the presented method, respectively.}
%     \label{fig:fullvslimited}
% \end{figure}

\begin{figure}[!ht]
\centering
\includegraphics[width=0.5\textwidth]{images/full_vs_limited_comparison.jpg}
\quad
\centering
\begin{tabular*}{0.5\textwidth}{@{}lllll@{}}\toprule
Method & \begin{tabular}[c]{@{}l@{}}Semantic \\ Label\end{tabular} & \begin{tabular}[c]{@{}l@{}}Semantic \\ Instance\end{tabular} & \begin{tabular}[c]{@{}l@{}}Temporal \\ Instance\end{tabular} \\ \midrule
    Limited Movement &   0.747   &    0.675    &  0.623  \\ 
    Full Movement    &   0.859   &    0.837    &  0.650  \\ \bottomrule
\end{tabular*}
\captionlistentry[table]{A table beside a figure}
\caption{A comparison of full vs limited movement schemes. The limited movement variant leads to significant drop in performance. In qualitative comparison (a) is the source scene with instance segmentation. (b) is the target scene visualization. (c) and (d) show result using our method using limited movement and result using full version of the presented method, respectively.}
\label{fig:fullvslimited}
\end{figure}

%  SEMANTIC LABEL
% FULL              (0.900 + 0.950 + 0.853 + 0.792 + 0.799) / 5 = 0.859
% LIMITED           (0.786 + 0.954 + 0.647 + 0.753 + 0.596) / 5 = 0.747

%  SEMANTIC INSTANCE
% FULL             (0.899 + 1.000 + 0.791 + 0.723 + 0.770) / 5 = 0.837
% LIMITED          (0.734 + 1.000 + 0.538 + 0.644 + 0.459) / 5 = 0.675



==> figures/inssegtable.tex <==
\begin{table*}[]
    \centering
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|}
    \hline
                   & \multicolumn{1}{l|}{Average} & \multicolumn{1}{l|}{chair} & \multicolumn{1}{l|}{sofa} & \multicolumn{1}{l|}{table} & \multicolumn{1}{l|}{desk} & \multicolumn{1}{l|}{other}  \\ \hline
    Rescan         & 0.849 & 0.899 & 1.000 & 0.816 & 0.770 & 0.763  \\ \hline
    MASC           & 0.291 & 0.370 & 0.396 & 0.153 & 0.124 & 0.414  \\ \hline
    \end{tabular}
    \caption{Semantic Instnace segmentation task. We report AP50\% scores for dynamic object classes }
    \label{tab:ins_seg_table}
\end{table*}

==> figures/multires.tex <==
\begin{figure}[b!]
    \centering
    \includegraphics[width=0.5\textwidth]{images/multires.jpg}
    \captionof{figure}{Multi-resolution pointcloud representation used in our method. Surfels are scaled up to better represent the surface at coarser levels.}
    \label{fig:multires}
\end{figure}


==> figures/semsegtable.tex <==
\begin{table*}[]
    \centering
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|}
    \hline
                 & \multicolumn{1}{l|}{Average} & \multicolumn{1}{l|}{chair} & \multicolumn{1}{l|}{sofa} & \multicolumn{1}{l|}{table} & \multicolumn{1}{l|}{desk} & \multicolumn{1}{l|}{other}  \\ \hline
    Rescan         & 0.8642 & 0.902 & 0.947 & 0.889 & 0.792 & 0.791  \\ \hline
    MASC           & 0.3108 & 0.516 & 0.325 & 0.160 & 0.242 & 0.311  \\ \hline
    SparseConvNet  & 0.2034 & 0.457 & 0.279 & 0.155 & 0.029 & 0.097   \\ \hline
    \end{tabular}
    \caption{Semantic segmentation results on the rescan dataset. We showcase the mean IoU semantic segmentation results on the dynamic object classes.}
    \label{tab:sem_seg_table}
\end{table*}
